Actionwave: A Systematic Benchmark for Waveform-Centric Clinical Prediction Across Care Scenarios

Continuous bedside waveforms record rapid physiological changes that can inform clinical decisions. Existing benchmarks examine selected prediction conditions, but it remains unclear how model advantages depend on signal duration, warning time, and available inputs across care settings. We introduce Actionwave, a benchmark for waveform-centric clinical prediction across intensive-care, operating-room, and emergency-department settings. Actionwave uses a common decision-time prediction interface and groups clinically grounded tasks by what is inferred and when. It varies conditions relevant to clinical use, including the warning required before an intervention. We compare diverse architectures and pretrained biosignal encoders under specified model-size and compute budgets. The protocol requires patient-level splits, strict information cutoffs, and comparisons that isolate individual modeling factors. Across 20 tasks and 1.4M task-labelled windows from source datasets, the experimental grids account for over 87,000 model fits. These comparisons identify task-specific choices and show why matched cohorts, unimodal controls, and explicit timing are necessary when interpreting waveform model performance.

==> iclr2026_conference.tex <==
% Compatibility entry point; edit and compile main.tex for the modular paper.
\input{main.tex}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/benchmark.tex <==
\section{Benchmark Definition}
\label{sec:formulation}

\noindent\textbf{Prospective prediction interface.}
Each benchmark example is a prospective episode
\(\mathcal{E}=(d,s,i,T,W,C,G,H,Y,M)\), where \(d\), \(s\), and \(i\) identify
the dataset, care setting, and patient-level split unit. At prediction time
\(T\), the model observes channels \(C\) over \([T-W,T)\); a future endpoint
\(Y\) is evaluated over \([T+G,T+G+H)\). The masks \(M\) distinguish absent or
invalid inputs, unascertained labels, and observed negative outcomes. Each task
contract fixes these fields together with its eligibility and label rules.

\noindent\textbf{Task organization.}
Clinical-inference labels provide descriptive context---acute safety-boundary
transition, pathophysiology or organ dysfunction, functional reserve or
intervention response, and trajectory or care disposition---but do not enter
model comparison or aggregation. Temporal geometry is part of the task
contract and distinguishes surveillance, gapped forecasts, event- or
daily-anchored predictions, and concurrent held-out-state probes. Direct task
comparisons require aligned labels, eligibility, input availability, and
temporal geometry. Full definitions and task assignments are provided in
Appendix~\ref{app:benchmark-taxonomies}.

\noindent\textbf{Evaluation contract.}
Within each task, we measure efficacy through discrimination and calibration,
efficiency through runtime, throughput, utilization, and memory, and
safety-relevant reliability through nonfinite behavior and prediction
collapse. Results are summarized across five seeds and then aggregated only
over matched task--model comparisons using equal-task macro averages;
final-model uncertainty uses patient-block bootstrap intervals. Detailed
metrics and aggregation rules appear in Appendix~\ref{app:evaluation-details}.

\section{Datasets and Task Construction}
\label{sec:data-task-construction}

This section establishes the stable evaluation population required for
controlled comparison. We first harmonize the three source datasets and then
construct frozen episodes with explicit eligibility, split, missingness, and
leakage rules. Keeping these decisions upstream of model evaluation prevents
temporal interventions from silently changing the comparison cohort; when an
eligibility change is unavoidable, its support and prevalence are reported.

\subsection{Dataset Overview}
Table~\ref{tab:dataset-summary} summarizes the three care settings before task-specific eligibility filtering.
Across datasets, preprocessing preserves physical time relative to the prediction anchor, uses a frozen dataset-specific resampling pipeline, retains channel-presence and sample-validity masks, and fits normalization statistics or learned quality filters on the training partition only.
The following paragraphs provide a compact introduction to each dataset.
Cohort, preprocessing, task, and development-support details are reported in
Appendix~\ref{app:dataset-details}, while full episode-construction and
data-control rules appear in Appendix~\ref{app:episode-data-controls}.

\begin{table*}[!t]
\centering
\scriptsize
\setlength{\tabcolsep}{4.0pt}
\renewcommand{\arraystretch}{1.12}
\caption{Compact dataset summary under the frozen benchmark preprocessing.
Patient counts precede task-specific filtering, and split ratios are training/validation/test.
ABP denotes arterial blood pressure, PPG denotes plethysmography, and RESP denotes respiration.}
\label{tab:dataset-summary}
\begin{tabular}{@{}lllllll@{}}
\toprule
Dataset & Setting & Patients & Split & Rate & Missingness & Channels \\
\midrule

MIMIC-III
& ICU
& 10,282
& 80/10/10
& 125\,Hz
& Variable
& ECG, ABP, PPG, RESP \\

\addlinespace
VitalDB
& Operating Room
& 6,090
& 70/15/15
& Native 62.5--500\,Hz
& Sparse; explicitly masked
& 12 waveform streams \\

\addlinespace
MC-MED
& ED
& 70,545
& 78/11/11
& Native
& Variable
& ECG-II, PPG, RESP \\

\bottomrule
\end{tabular}
\end{table*}

\noindent\textbf{MIMIC-III.}
% \label{sec:data-mimic}
The MIMIC-III Waveform Database Matched Subset~\citep{moody2020mimic3waveform} provides 125\,Hz ICU waveforms linked to clinical records for 10,282 adults.
Its variably available ECG, arterial-pressure, plethysmography, and respiration channels support eight tasks spanning deterioration, organ dysfunction, treatment-response proxies, and episode outcomes.
We use a frozen 80/10/10 patient-level split and preserve channel-presence and validity masks; complete task definitions are given in Appendix~\ref{app:mimic-details}.

\noindent\textbf{VitalDB.} % @Davis
% \label{sec:data-vitaldb}
VitalDB~\citep{lee2022vitaldb} contains high-resolution intraoperative waveforms and numeric tracks from 6,090 patients across 6,388 surgical cases under a frozen 70/15/15 subject-level split.
The waveform-only benchmark uses twelve permitted waveform streams sampled at 62.5--500\,Hz, while numeric and laboratory tracks are reserved for eligibility and outcome construction.
These signals support seven future-event tasks and one concurrent held-out-state probe; preprocessing and endpoint definitions are detailed in Appendix~\ref{app:vitaldb-details}.

\noindent\textbf{MC-MED.}
% \label{sec:data-mcmed}
MC-MED~\citep{kansal2025mcmed} contains 70,545 adult ED patients across 118,385 visits and uses the supplied 78/11/11 chronological, patient-disjoint split; completed representation-comparison test results are reported in Figure~\ref{fig:representation-results}.
Waveform sampling rates are channel-dependent, and ECG lead II, plethysmography, and respiration are intermittently available.
We select four tasks: 60-minute physiological decompensation, pending hyperkalemia, lactate nonclearance, and pending severe anemia.
Laboratory outcomes are assessed up to 240 minutes after prediction, with repeat lactate restricted to 30--240 minutes.
Task definitions and waveform coverage are reported in Appendix~\ref{app:mcmed-details}; task-specific training and validation support is reported in Table~\ref{tab:mcmed-task-support}.

\subsection{Episode Construction and Data Controls}
\label{sec:episode-data-controls}

\noindent\textbf{Episode construction and eligibility.}
Each task defines candidate decision anchors \(T\) and materializes the
observation interval \([T-W,T)\), optional forecast gap \(G\), and outcome
horizon \(H\) independently of future labels. For incident-event tasks,
eligibility excludes prevalent events and requires enough follow-up and target
availability to distinguish positive, negative, and unascertained outcomes;
missing or incomplete outcomes remain masked rather than being treated as
negative. Dataset-specific anchor families, gap handling, response-task rules,
and repeated-episode handling are detailed in
Appendix~\ref{app:episode-data-controls}.

\noindent\textbf{Splits, missingness, and leakage control.}
% \label{sec:data-splits-leakage}
Subjects are partitioned before inputs are constructed, and no subject
contributes waveforms or anchors to more than one split. Frozen preprocessing
retains channel-presence and sample-validity masks, while normalization and all
learned preprocessing are fit on training subjects only. Inputs must precede
the decision-time cutoff, and post-anchor, outcome-derived, label, censoring,
and direct target features are excluded. The complete preprocessing,
availability, exclusion, and audit rules are provided in
Appendix~\ref{app:episode-data-controls}.


==> sections/experiment.tex <==
\section{Controlled Experimental Design}
\label{sec:benchmark}

Building on the episodes in Section~\ref{sec:data-task-construction}, the experimental design addresses the two confounds and two underexplored variation axes through a shared comparison protocol.
Every experiment uses the same subject splits and validation and test partitions, five model seeds, and matched parameter, token, optimization, and search budgets wherever possible; except when task formulation is varied, conditions also share eligible episodes, anchors, labels, observation bounds, channels, and missingness masks.
These controls make differences attributable to the declared intervention and operationalize the \textit{Common task contract} and \textit{Multidimensional evaluation} while preserving the \textit{Clinical inference target} and \textit{Temporal geometry} whenever they are not under study.
Table~\ref{tab:benchmark-comparison} summarizes how this scope extends the comparison dimensions covered by existing benchmarks.

\noindent\textbf{Representation and Architecture Interventions.}
We first compare raw strided stems, fixed and multiscale patches, spectral tokens, and beat- or pulse-aligned tokens over the same interval and channels, then vary mask-aware and learned missing-value handling under the selected tokenizer; all preprocessing and imputation models are fit on training subjects only and evaluated primarily by downstream utility.
Using the resulting prespecified input pipeline, we compare ConvNet, TCN, Transformer, S4, Mamba, and compatible pretrained biosignal encoders on the same episodes and inputs within a declared parameter band, marking unsupported pretrained configurations as N/A.
This staged comparison isolates representation, missing-data, and architecture effects instead of attributing tokenizer, channel, or scale differences to the encoder.
It therefore directly addresses the frontend--encoder confound through \textit{Controlled interventions} under the \textit{Common task contract}.

\noindent\textbf{Task-Formulation Interventions.}
We vary observation length and forecast gap separately using nested waveform suffixes, a common legal cutoff, and the contracts in Section~\ref{sec:episode-data-controls}; for each gap, we report eligibility, prevalence, and follow-up support.
The design measures the value of additional context and warning time without silently conflating them with avoidable cohort changes.
It directly tests \textit{Task-formulation variation} along the \textit{Temporal geometry} axis and addresses the eligibility, cohort-composition, and prevalence confound.

\noindent\textbf{Deployment, Data, and Modality Interventions.}
We compare channel-selection policies at budgets of 2, 4, and 8 channels, apply prespecified inference-time dropout stress tests, and evaluate bidirectional source-domain transport only for aligned endpoints, channels, and temporal geometry; unselected channels remain masked, and target test labels are never used for selection.
These experiments quantify sensing burden, failure under missing inputs, and transportability across patient and practice distributions.
We also vary the number of unique training subjects while keeping validation and test sets fixed across subset seeds, reporting the full learning curve and the smallest budget recovering 90\% of full-data performance.
On aligned episodes, waveform-only and EHR-only baselines are compared with early, late, cross-attention, and gated fusion, and fusion must improve on the stronger unimodal baseline after accounting for compute and missing-input robustness.
Together, these \textit{Controlled interventions} test \textit{Deployment-context variation} across sensor access, source domains, training data availability, and modalities while preserving the \textit{Clinical inference target} and \textit{Temporal geometry}.

\noindent\textbf{Incremental Evaluation and Reproducibility.}
Experiments advance through prespecified validation-gated stages, sealed test results are evaluated once after each comparison is locked, and every run records its configuration, seed, fold, code revision, data hashes, and checkpoint.
Models share the optimizer, stopping, search, update, and hardware protocols wherever applicable.
The full promotion path remains auditable, and later system comparisons retain clear attribution to earlier decisions without test-set feedback.
The schedule enforces \textit{Controlled interventions} within the \textit{Common task contract} and carries their efficacy, efficiency, and safety consequences into \textit{Multidimensional evaluation}.

\section{Experiment Results}
\label{sec:results}
We evaluate waveform-only models on eight MIMIC-III, eight VitalDB, and four MC-MED tasks, encoding unavailable channels as NaN with binary masks without complete-case filtering. Figure~\ref{fig:representation-results} compares (a) nine encoders at a matched $\sim$500k-parameter budget with three tokenizers and (b) seven tokenizers with a fixed Transformer backbone. Models use five seeds, with learning rates and, in part~(a), tokenizers selected by validation AUROC only. We report test AUROC as the mean and sample standard deviation across seeds, with equal-task macro averages; VitalDB's concurrent-state probe is reported separately from its forecast macro. Panel~(c) reports Crossformer and SeFT contrasts against Conv1D for MIMIC-III and VitalDB, and Conv2D contrasts against Conv1D for MC-MED. All three datasets have completed figure results; exact MC-MED per-method means and seed SDs remain to be tabulated. The detailed MIMIC-III and VitalDB scores are given in Appendix~\ref{app:representation-results}, Table~\ref{tab:main_auroc}; task definitions, preprocessing, model grids, training settings, and selection and aggregation rules are provided in Appendix~\ref{app:architecture-tokenizer-protocol}.

\subsection{Architecture--Tokenizer Comparison}
\label{sec:architecture-tokenizer-comparison}

We first compare eligible architecture--tokenizer pairs using a common five-minute waveform view.
All configurations use the same eligible episodes, subject folds, task-permitted channels, missingness representation, train-fold-only normalization, optimization budget, and evaluation protocol.
Architecture widths are adjusted to remain within the declared parameter band, and differences in token count or computational cost are reported explicitly.
Validation task wins determine the architecture--tokenizer pairs carried forward to the observation-length comparison.


\subsection{Input-length Comparison}
\label{sec:input-length-comparison}

Following the benchmark factorization in Section~\ref{sec:benchmark}, we analyze observation length and forecast gap as separate benchmark perturbations.
Observation-length comparisons first restrict the cohort to episodes satisfying the longest-history eligibility requirement.
Shorter inputs are then constructed as nested waveform suffixes ending at the same prediction anchor, preserving the endpoint, gap, horizon, eligible episodes, subject split, channel policy, and all other model settings.
Forecast-gap changes may alter prevalence, support, and cohort membership, so these axes are analyzed separately.

These temporal choices encode task-specific clinical requirements.
Prior work has evaluated intraoperative hypotension prediction 5, 10, and 15 minutes before onset, with discrimination varying across these lead times~\citep{hatib2018machine,lee2021deep}, whereas the PhysioNet 2019 sepsis challenge targeted prediction six hours before clinical recognition~\citep{reyna2020early}.

\paragraph{Observation length.}
We evaluate nested waveform histories of 5, 15, 30, and 60 minutes for Transformer/patch, S4/patch, S4/SeFT, BiLSTM/patch, and DLinear/patch.
These five architecture--tokenizer pairs were retained from the preceding validation comparison under the prespecified task-win and tie policy; no test result was used to break the validation ties.
Within each task and forecast gap, all context-length conditions use the same 60-minute-eligible episodes, labels, subjects, and outer folds.
Each view ends at the same legal cutoff, and shortening the context removes only the oldest waveform samples.
We report equal-task AUROC and AUPRC, task wins, proper scores, seed and fold dispersion, and a block-order-permuted control that distinguishes temporal-order effects from the benefit of receiving more waveform samples.

\paragraph{Forecast gap.}
Across the seven VitalDB future-event tasks, increasing the blank gap from five to 15 minutes changes waveform-only AUROC by \result{gap result} and AUPRC by \result{gap result}.
Absolute performance \result{decreases/remains stable/varies by task}.
Because changing the gap also changes which events and subjects remain eligible, Figure~\ref{fig:temporal} reports task-level prevalence and positive-subject support at each gap.
We additionally evaluate the intersection of examples eligible under both gaps as a matched sensitivity analysis; this yields \result{matched-cohort result}.
The concurrent BIS task is excluded from these aggregates because it estimates a simultaneous held-out state rather than a future event.
MIMIC-III gap sensitivities are reported separately at their task-native hourly geometries and are not pooled with the minute-scale operating-room forecasts.

\begin{figure*}[!t]
\centering
\includegraphics[width=\textwidth]{figures/figurer1_placeholder.png}
\vspace{-6mm}
\caption{Temporal interventions shown as context-length and forecast-gap comparisons.
Shorter context windows use nested waveform suffixes from the same longest-history-eligible episodes.
\textbf{Placeholder only: all displayed values are synthetic and must be replaced by locked outputs.}}
\label{fig:temporal}
\end{figure*}


\subsection{Whole-subject Selection and Data Efficiency}
\label{sec:whole-subject-selection}

The data budget is the number or fraction of unique subjects available for training.
Figure~\ref{fig:data_efficiency} compares random, prevalence-stratified, and representation-diverse subject selection at matched fractions of the training cohort.
Selection is performed once per seed at the subject level; all episodes from a selected subject are then available for training, while the validation and test cohorts remain unchanged.
At \result{best reduced data budget}, \result{best selection method} improves the equal-task metric by \result{data-selection gain} over random selection and reaches 90\% of full-data performance with \result{number or fraction of subjects}.
The gain is \result{largest or smallest} on tasks with few positive subjects, while \result{method or condition} has the lowest variance across subset seeds.

Performance does not increase uniformly with the number of waveform fragments: subject diversity and positive-subject support explain \result{data-efficiency finding} beyond the raw episode count.
We therefore report both subjects and episodes at every budget.
Selection methods and data-efficiency thresholds are chosen using validation data only; locked test results assess whether the prespecified conclusion holds, with calibration, subgroup, and rare-task guardrails reported alongside it.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/data_efficiency_placeholder.png}
\vspace{-6mm}
\caption{Whole-subject data efficiency across subset-selection methods, with uncertainty across seeds and the sample size required to recover 90\% of full-data performance.
\textbf{Placeholder only: all displayed values are synthetic and must be replaced by locked outputs.}}
\label{fig:data_efficiency}
\end{figure}


\subsection{Channel-selection Policy and Sensing Budget}
\label{sec:channel-selection}

We compare five training-only channel selectors---mutual information, L1/lasso, waveform SQI, temporal mutual information, and random selection---at 2-, 4-, and 8-channel budgets, together with an all-permitted-channel comparator.
The comparison uses the same Core-8 episodes, subject folds, five-minute model views, normalization contexts, and the frozen Transformer/patch, Mamba3/patch, and Transformer/Crossformer architecture--tokenizer pairs inherited from the channel-selection protocol.
Selector scores are estimated exclusively from the four outer-training folds; held-fold and sealed-test subjects are never used to score or rank channels.

All conditions retain the same 66-slot input geometry.
Missing and unselected streams remain NaN with mask value false, and no episode is removed because a selected sensor is unavailable.
For VCS05, EEG1 and EEG2 are removed from the candidate set before selection.
We report equal-task AUROC and AUPRC, proper scores, task wins, selection stability across seeds and folds, and the smallest channel budget that retains \result{prespecified percentage} of full-panel performance.
These comparisons estimate predictive sufficiency under a sensing budget and are not interpreted as causal estimates of channel importance.

\subsection{Missing-Channel Handling and Imputation}
\label{sec:missing-channel-results}

We evaluate ten missing-channel strategies at a fixed five-minute context for Transformer/patch, Mamba-3/patch, and Transformer/Crossformer.
The comparison includes architecture-only handling, zero filling with a mask and time-since-observed feature, GRU-D, lead-agnostic self-supervision, Rectified Flow, TrigFlow, Drifting Model, GRIN, Raindrop, and positional kriging.
Every condition uses the same task cohorts, subject folds, legal input cutoffs, and canonical 66-slot geometry.
Learned components are fit using subjects from the four outer-training folds only.

Natural VitalDB channel availability is the primary comparison.
We separately evaluate prespecified inference-only stress conditions using deterministic 25\% and 50\% observed-channel dropout and modality-group dropout.
These stress masks do not alter training, eligibility, or method selection.
We report equal-task AUROC and AUPRC, Brier score, log loss, expected calibration error, task wins, seed and fold dispersion, and computational efficiency.
The seven future-event tasks and concurrent VCS05 probe are additionally summarized separately, with uncertainty estimated using 2,000 paired whole-subject bootstrap draws.

On validation, \result{best overall method and macro AUROC/AUPRC}, while \result{most consistent method} records \result{task-win or dispersion result}.
Under controlled channel dropout, \result{robustness finding}.
Generative approaches \result{performance and efficiency comparison}, whereas \result{competitive non-generative methods} provide \result{efficacy--efficiency finding}.
All ten prespecified methods are retained through the locked comparison; sealed-test outcomes are not used to reorder, modify, or prune the panel.

\subsection{Waveform-centric Fusion}
In the completed three-task MIMIC-III comparison of acute deterioration, circulatory deterioration, and respiratory escalation, the best mixture-of-experts configuration reaches a mean headline metric of approximately \(0.81\) at \(9.8\times10^{-3}\) GFLOPs per example.
This exceeds the strongest evaluated full-window fusion alternative (approximately \(0.793\)), as well as the tabular-only (\(0.763\)) and waveform-only (\(0.739\)) experts.
Thus, the observed gain is not an artifact of comparison with only one weak modality and lies on the efficacy versus compute frontier of the 24 evaluated methods.

The benefit does not extend automatically to combining missing-waveform imputers.
On the same task subset, neither an early-fusion MoE router nor a late-fusion stacker outperforms the best individual imputer on any of the three tasks.
These results support separate promotion rules for multimodal fusion and imputer ensembling: each candidate must beat its strongest constituent at matched episodes and report its incremental compute.
The full 20-task analysis will apply this locked rule and report \result{aggregate fusion gain}, \result{calibration change}, and \result{missing-modality retention} once all test outputs are available.

\begin{figure*}[!t]
\centering
\includegraphics[width=\textwidth]{figures/mimic result fig.png}
\vspace{-6mm}
\caption{SYNTHETIC: Waveform-centric fusion results on the completed MIMIC-III task subset, showing predictive performance and compute for waveform-only, EHR-only, and multimodal configurations.}
\label{fig:mimic-fusion}
\end{figure*}

\subsection{Out-of-Distribution Evaluation}

\begin{figure*}[!t]
\centering
\includegraphics[width=\textwidth]{figures/transport_data_budget_placeholder.png}
\vspace{-6mm}
\caption{Cross-setting transport on homologous tasks and common sensors, showing directional domain regret, calibration, and adaptation with limited target-domain training data.
\textbf{Placeholder only: all displayed values are synthetic and must be replaced by locked test outputs.}}
\label{fig:transport}
\end{figure*}

\subsection{Efficacy, Efficiency, and Safety-relevant Trade-offs}


==> sections/introduction_draft.tex <==
\section{Introduction}

\begin{wrapfigure}{r}{0.25\textwidth}
    \centering
    \vspace{-\intextsep}
    \includegraphics[width=\linewidth]{figures/benchmark_design_philosophy.pdf}
    \vspace{-7mm}
    \caption{\small \method: clinically grounded tasks and controlled comparisons provide evidence to guide future model development.}
    \label{fig:design-philosophy-draft}
    \vspace{-6mm}
\end{wrapfigure}
    
Continuous bedside monitoring captures physiological dynamics that intermittent clinical measurements cannot fully represent.
Electrocardiography, arterial blood pressure, photoplethysmography, and respiration record changes over seconds to minutes, providing a rich basis for clinical prediction.
Their predictive value, however, depends on the conditions under which a prediction is made.
Intensive-care units, operating rooms, and emergency departments differ in available sensors, monitoring duration, and the warning time required before an intervention.
A systematic understanding of these conditions can guide the development of clinical waveform models by identifying which design choices are effective, where their benefits persist, and which limitations require further methodological progress.

Recent advances in waveform encoders and biosignal foundation models have expanded the approaches available for clinical prediction.
Benchmarks such as YAIB, MC-BEC, and SignalMC-MED have strengthened reproducible evaluation and examined important variations in clinical definitions, modalities, and signal duration~\citep{vandewater2024yaib,chen2023mcbec,gustafsson2026signalmcmed}.
Nevertheless, determining which raw-waveform modeling choices yield consistent advantages across care settings and prediction conditions remains difficult.
Two confounds complicate this assessment.
First, encoder comparisons often also change tokenization, sampling, input channels, or computational resources, making architectural gains difficult to separate from differences in the input representation.
Second, changing observation length or forecast gap can alter episode eligibility, follow-up availability, and outcome prevalence.
Consequently, performance differences may reflect changes in the prediction population or task difficulty alongside the modeling factor under investigation.
Interpretable comparisons therefore require explicit control over both the information provided to models and the construction of prediction tasks.
Table~\ref{tab:benchmark-comparison-draft} positions our combination of raw-waveform, multi-source task coverage and experimental axes relative to complementary benchmarks.

\begin{table}[!t]
\centering
\caption{Comparison with clinical time-series and waveform benchmarks, with experimental axes grouped by our three research questions.
Scope columns indicate dataset/task coverage; RQ columns indicate explicit comparisons (\yesicon{}) or no separately reported comparison (--).
The \method{} row summarizes the specified benchmark design.}
\label{tab:benchmark-comparison-draft}
\label{tab:benchmark-comparison}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}l*{9}{c}@{}}
\toprule
& \multicolumn{3}{c}{\textbf{Scope}}
& \multicolumn{1}{c}{\textbf{RQ1}}
& \multicolumn{2}{c}{\textbf{RQ2: Time}}
& \multicolumn{3}{c}{\textbf{RQ3: Information}} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-5}\cmidrule(lr){6-7}\cmidrule(l){8-10}
Benchmark
& Raw waveform
& Multiple sources
& Multiple tasks
& Tokenization
& Observation length
& Gap or horizon
& Input panels
& Missingness
& Data budget \\
\midrule
MIMIC-III Benchmark~\citep{harutyunyan2019multitask}
& -- & -- & \yesicon
& -- & -- & -- & -- & -- & -- \\
\addlinespace[1pt]
YAIB~\citep{vandewater2024yaib}
& -- & \yesicon & \yesicon
& -- & -- & -- & \yesicon & -- & \yesicon$^{\dagger}$ \\
\addlinespace[1pt]
PulseDB~\citep{wang2023pulsedb}
& \yesicon & \yesicon & --
& -- & -- & -- & -- & -- & -- \\
\addlinespace[1pt]
MC-BEC~\citep{chen2023mcbec}
& \yesicon & -- & \yesicon
& -- & -- & \yesicon & \yesicon & \yesicon & -- \\
\addlinespace[1pt]
MDS-ED~\citep{lopezalcaraz2025enhancing}
& \yesicon & -- & \yesicon
& -- & -- & -- & \yesicon & \yesicon$^{\ddagger}$ & -- \\
\addlinespace[1pt]
SignalMC-MED~\citep{gustafsson2026signalmcmed}
& \yesicon & -- & \yesicon
& -- & \yesicon & -- & \yesicon & -- & \yesicon \\
\midrule
\method{} (ours)
& \yesicon & \yesicon & \yesicon
& \yesicon & \yesicon & \yesicon & \yesicon & \yesicon & \yesicon \\
\bottomrule
\end{tabular}%
}
\vspace{-6mm}
\end{table}

We organize our study around three research questions, each connected to a concrete decision in clinical waveform model development:
\begin{tcolorbox}[
    colback=black!5!white,
    colframe=black!55!white,
    boxrule=0.4pt,
    arc=1.5pt,
    left=5pt,
    right=5pt,
    top=3pt,
    bottom=3pt
]
\textbf{(RQ1) Representation and architecture.}
How do waveform tokenization and encoder choices affect predictive performance and model rankings under controlled comparisons?
\par\smallskip
\textbf{(RQ2) Temporal modeling.}
How do observation history and required warning time affect predictability, accounting for changes in episode eligibility and outcome prevalence?
\par\smallskip
\textbf{(RQ3) Information availability.}
When do additional sensors, training subjects, and clinical modalities improve prediction, and how robust are these gains to missing inputs?
\end{tcolorbox}

To investigate these questions, we introduce \method{} (Figure~\ref{fig:design-philosophy-draft}), a waveform-centric benchmark defining 20 tasks across MIMIC-III intensive-care records, VitalDB surgical records, and MC-MED emergency-department records~\citep{moody2020mimic3waveform,lee2022vitaldb,kansal2025mcmed}.
Each task specifies its prediction anchor, observation window, forecast gap, target horizon, permitted inputs, and eligibility rules, with concurrent state-estimation probes evaluated separately from future-event forecasts.
Patient-disjoint splits and explicit information cutoffs support controlled comparisons of representations, temporal formulations, and information availability.
Evaluation considers discrimination, calibration, computational cost, and robustness, with patient-level uncertainty and transparent reporting of cohort changes.
These comparisons are designed to identify effective modeling choices, characterize their operating limits, and expose unresolved challenges in temporal modeling and multimodal integration.
By connecting empirical findings to concrete design decisions, \method{} aims to provide the community with evidence-based guidance for developing future clinical waveform models, supported by explicit task definitions and reproducible evaluation protocols.

